Mirrored Langevin Dynamics

We consider the problem of sampling from constrained distributions, which has posed significant challenges to both non-asymptotic analysis and algorithmic design. We propose a unified framework, which is inspired by the classical mirror descent, to derive novel first-order sampling schemes. We prove that, for a general target distribution with strongly convex potential, our framework implies the existence of a first-order algorithm achieving $\tilde{O}(\epsilon^{-2}d)$ convergence, suggesting that the state-of-the-art $\tilde{O}(\epsilon^{-6}d^5)$ can be vastly improved. With the important Latent Dirichlet Allocation (LDA) application in mind, we specialize our algorithm to sample from Dirichlet posteriors, and derive the first non-asymptotic $\tilde{O}(\epsilon^{-2}d^2)$ rate for first-order sampling. We further extend our framework to the mini-batch setting and prove convergence rates when only stochastic gradients are available. Finally, we report promising experimental results for LDA on real datasets.

==> app_W_nonconvex.tex <==
\section{W is Non-Convex when $\dV$ is Exponential/Gaussian and $h$ is Burg's Entropy}\label{app:W_nonconvex}
In dimension 1, let $V(x) = x$ and $h(x) = -\log x$ (known as the Burg's entropy function) where $x \in (0,\infty)$. Then $\hstar (y) = - \log (-y) -1$ on $(-\infty, 0)$. Plugging these terms into \eqref{eq:Monge-Ampere-dual} yields 
\beq \nn
W(y) = -\frac{1}{y} + 2\log (-y), \quad y<0.
\eeq
We have $W''(y) = \frac{-2-2y}{y^3}$, which is negative when $y< -1$.

Similarly, when $V(x) = c x^2$ for some normalizing $c$ and $x > 0$, we have
\beq \nn
W(y) = \frac{c}{y^2} + 2\log (-y), \quad y<0.
\eeq
Hence $W''(y) = \frac{6c-2y^2}{y^4}$, which is negative when $y< -\sqrt{3c}$.

==> app_asymmetric_sde_x.tex <==
\section{Stochastic Differential Equation of $\X_t$ for Asymmetric Mirrored Langevin Dynamics}\label{app:A-MLD_SDE_X}
We show that the A-MLD
\beq \label{eq:app_A-MLD}
   \left\{
                \begin{array}{ll}
                  \drm\Y_t = -(\nabla W\circ \nabla h)(\X_t) \dt + \sqrt{2} \dBt\\
                  \X_t = \nabla \hstar (\Y_t)
                \end{array}
        \right.
\eeq
incurs the following SDE on $\X_t$.

\begin{theorem}
Let $\X_t$ and $\Y_t$ be as in \eqref{eq:app_A-MLD}. Then the SDE governing $\X_t$ is
\beq\label{eq:app_A-MLD_vu} 
\drm \X_t = v(\X_t)\dt + u(\X_t)\dBt,
\eeq
where 
\beq  \nn
   \left\{
                \begin{array}{ll}
                  u = \nabla^2 h^{-1}\\
                  v = -\nabla^2 h^{-2} \l( \nabla V + \nabla \log \det \nabla^2 h \r) - \textup{vec}\l(\Tr\nabla^2 h^{-2} \nabla^2(\partial_i h) \r),
                \end{array}
        \right.
\eeq
where $\textup{vec}(z_i)$ vectorizes the scalars $z_i$'s.
\end{theorem}
\begin{proof}
Applying It\^o's lemma to $\nh$ in \eqref{eq:app_A-MLD_vu} gives
\beq \label{eq:app_A-MLD_hold1}
\drm \Y_t = \l(  \nabla^2 h(\X_t) v(\X_t) + \textup{vec}\l(\Tr u(\X_t)u(\X_t)^\top \nabla^2 (\partial_i h) \r)\r)\dt + \sqrt{2} \nabla^2 h(\X_t) u(\X_t) \dBt.
\eeq
Equating \eqref{eq:app_A-MLD_hold1} with \eqref{eq:app_A-MLD} yields
\beq \label{eq:app_A-MLD_vu_hold}
   \left\{
                \begin{array}{ll}
                  u \cdot\nabla^2 h= I\\
                    \nabla^2 h(\X_t) v(\X_t) + \textup{vec}\Big(\Tr u(\X_t)u(\X_t)^\top \nabla^2 (\partial_i h) \Big)= - \nabla W \circ \nh.
                \end{array}
        \right.
\eeq
By \eqref{eq:Monge-Ampere}, we have
\beq \label{eq:app_A-MLD_hold2}
\nabla^2 h \cdot (\nabla W \circ \nh) = \nabla V + \nabla \log \det \nabla^2 h.
\eeq
The proof is finished by using \eqref{eq:app_A-MLD_hold2} in \eqref{eq:app_A-MLD_vu_hold} and straightforward calculations.
\end{proof}

==> app_cir.tex <==
\section{Symmetric Mirrored Langevin Dynamics Covers Cox–Ingersoll–Ross Processes}\label{app:cir}
Let $a,b$, and $c$ be given positive numbers such that $2ab \geq c^2$. This corresponds to an interesting regime of the Cox–Ingersoll–Ross Processes \citep{brigo2007interest} in dimension 1:
\beq \label{eq:cir_process}
\drm X_t = a(b-X_t)\dt + c\sqrt{X_t}\drm B_t.
\eeq
We present a convex $V$ and a convex mirror map $h$ such that the S-MLD reduces to the Cox–Ingersoll–Ross Process.

Let $h(x) = \frac{2}{c^2} \cdot x\log x$ on $\RR^+$. Then $\sqrt{2h''(x)^{-1}} = c\sqrt{x}$. By the Monge-Amp\`ere equation \eqref{eq:Monge-Ampere}, we have
\begin{align*}
W \circ h' &= V + \log h''  \\
&=  V - \log x + \log \frac{2}{c^2}.
\end{align*}
Differentiating both sides yield
\begin{align*}
W' \circ h' &= \l(h''\r)^{-1} \l( V' - \frac{1}{x}\r) \\
&= \l(h''\r)^{-1}V'  - \frac{c^2}{2}.
\end{align*}
If $V' = \frac{2a}{c^2} + \l( 1- \frac{2ab}{c^2}\r) \frac{1}{x}$, that is when $V(x) = \frac{2a x}{c^2} + \l( 1-\frac{2ab}{c^2}\r) \log x + C$ for some normalizing constant $C$, then we get 
\beq \nn
(W' \circ h') (x)= a(x-b).
\eeq
Plugging this into \eqref{eq:sde_X}, we get \eqref{eq:cir_process}. Finally, notice that $V$ is convex since $2ab \geq c^2$.

==> app_convergence_smld.tex <==
\section{Proof of Theorem \ref{thm:convergence_conti_mld}}\label{app:proof_convergence_smld}
By \textbf{Corollary 4.2} of \citet{kolesnikov2014hessian}, the expressions given in \textbf{Appendix \ref{app:ricci}} coincides with the Bakry-\'Emery tensor. A classical result in the Bakry-\'Emery theory \citep{bakry2013analysis} states that if $\Ricg \succeq \rho \nabla^2 h$, then the following Poincar\'e inequality holds:
\beq \label{eq:poincare}
\Var_\mu\l(  P_t f \r) \leq e^{-2\rho t} \Var_\mu(f)  \quad \forall f\in\Cc
\eeq
where $P_t= e^{t\Lh}$ is the semigroup operator associated with the generator $\Lh$. The rest of the proof follows almost verbatim from Section A.2.1 of \citet{dalalyan2017theoretical}. We present a slightly different proof below for completeness.

%For the sake of completeness, we present a slightly different proof that \footnote{Notice that the $d_{\textup{TV}}$ in \citep{dalalyan2017theoretical} is $2d_{\textup{TV}}$ in our paper.}tightens the constant by 2.

Let $P_t^\star$ denote the operator acting on the set of measures $\mu_0$ via
\beq
\int P_t f  \drm\mu_0 = \int f \drm \l(P_t^\star\mu_0\r)  \quad \forall f\in \Cc.
\eeq 
Then $P_t^\star\mu_0$ is the law of $\X_t$.  Notice that $P_t^\star\mu = \mu$ for all $t>0$.

We now write, for $E$ a Borel set and $1_E$ being the indicator function of $E$,
\begin{align*}
d_{\textup{TV}} (\mu_t, \mu) &= d_{\textup{TV}} (P_t^\star\mu_0, \mu) \\
&=\sup_{E} | P_t^\star\mu_0 (E)- \mu(E)| \\
&=\sup_{E} \left|     \int  1_E    \drm (P_t^\star\mu_0 ) -    \int  1_E \drm (P_t^\star\mu )  \right| \\
&=\sup_{E} \left|    \int P_t  1_E    \drm \mu_0  -    \int  P_t 1_E \dmu \right| \\
&= \sup_{E} \left|     \int \  \l(P_t 1_E \r) \cdot \l( \frac{\dmu_0}{\dmu} -1\r)\dmu \right|  \\
&\leq \sup_{E}  \sqrt{   \int \  \l( P_t 1_E \r)^2 \dmu } \cdot \sqrt{ \int \l( \frac{\dmu_0}{\dmu} -1\r)^2\dmu }.
\end{align*}
By Jensen's inequality, we have $\l( P_t 1_E \r)^2 \leq P_t 1^2_E =   P_t 1_E $. Invoking the Poincar\'e inequality \eqref{eq:poincare}, we may write  
\begin{align*}
d_{\textup{TV}} (\mu_t, \mu) &\leq e^{-\frac{\rho t}{2}} \cdot\sqrt{\mu(E)\cdot \l(1-\mu(E)\r)}\cdot \sqrt{\chi^2(\mu_0, \mu)} \\
&\leq \frac{1}{2} \sqrt{\chi^2(\mu_0, \mu)}e^{-\frac{\rho t}{2}} 
\end{align*}which finishes the proof.

%
%\item By \citep{kolesnikov2014hessian}, $\Ricg$ is the Bakry-\'Emery tensor associated with the Riemannian manifold $(\RR^d, \nabla^2h, \mu)$. By \textbf{Theorem 5.7.4} and \textbf{5.2.1} of \citep{bakry2013analysis}, $\Ricg \succeq \rho \nabla^2 h$ implies  
%\beq
%\Ent_\mu (P_tf) \leq \Ent_\mu f \cdot e^{-2\rho t} \quad \forall f\in \Cc,
%\eeq \nn
%where $P_t$ is the semigroup \citep{bakry2013analysis} associated with $\Lh$, and $\Ent_\mu \coloneqq \int f\log f\dmu - \l(\int f\dmu \r) \log \l(\int f \dmu\r).$ Let $P_t^\star$ denote the operator acting on the set of measures $\mu_0$ via
%\beq
%\int P_t f  d\mu_0 = \int f \drm \l(P_t^\star\mu_0\r)  \quad \forall f\in \Cc.
%\eeq \nn
%Then $P_t^\star\mu_0$ is the law of $\X_t$. Then, letting $f\leftarrow \frac{\dmu_0}{\dmu}$, we get
%\begin{align*}
%D(P_t^\star\mu_0 \| \mu) = \int 
%\end{align*}

%\begin{table}
%\centering
%\caption{\label{tab:table_2D} PSNR and SSIM performances averaged on 60 test slices at 25\% subsampling rate. The entries where the learning is matched to the decoder and performance measure are shown in bold.   }
%\begin{tabular}{|l|||*{4}{c|}}\hline
%%\backslashbox{Mask}{Decoder}
%&\makebox[3em]{TV}&\makebox[3em]{BP}&\makebox[3em]{BM3D} &\makebox[3em]{{NN}} \\\hline \hline
%%TV-parametric & 29.87 &   29.54 &  31.49  & 28.14 \\\hline
%%BP-parametric &    29.73  & 29.46  & 31.25 & 28.20 \\\hline
%%BM3D-parametric &  29.08  & 28.71  & 32.88& 29.15 \\\hline
%%NN-parametric &  29.13   &   29.01 & 32.65 & 29.26\\\hline \hline
%Coherence-based &  30.76  &   31.48 & 30.04 & 32.02  \\\hline %30.32
%Single-image &  32.79   &   33.32 & 32.42 & 33.67 \\\hline \hline %32.41
%TV-greedy & {\bf 34.84} & 36.08 & 35.95 & 36.04  \\\hline %35.19
%BP-greedy & 34.76 &  {\bf 36.16} & 36.11 & 36.17 \\\hline  %35.04
%BM3D-greedy &  34.77 &  36.04 & {\bf 36.19}& 35.92 \\\hline %35.22
%% \rev{NN-greedy} &  34.67 &  35.85 &  35.92 & {\bf 35.26} \\\hline  % old values
%{NN-greedy} &  34.81 &  36.05 &  36.16 & {\bf 36.36} \\\hline %  35.26
%{Low Pass} &  31.96  &  32.41 & 32.59 & 32.59 \\\hline
%\end{tabular}
%
%\vspace{2mm}
%
%\begin{tabular}{|l|||*{4}{c|}}\hline
%%\backslashbox{Mask}{Decoder}
%&\makebox[3em]{{TV}}&\makebox[3em]{{BP}}&\makebox[3em]{{BM3D}} &\makebox[3em]{{NN}} \\\hline \hline
%
%
%{Coherence-based}&0.832&0.85&0.822  & 0.798  \\\hline
%{Single-image}&0.876&0.889&0.879   & 0.854  \\\hline
%{TV-greedy} &{ 0.907}&0.922&0.921  & 0.869  \\\hline
%{BP-greedy}&0.906& { 0.923}&0.921  & 0.859  \\\hline
%{BM3D-greedy}&0.906&0.922&{0.922}  & 0.909  \\\hline
%{NN-greedy}&0.907&0.923&0.923   & {0.925}  \\\hline
%{Low Pass}&0.876&0.888&0.893  & 0.893  \\\hline
%\end{tabular}
%\end{table}

==> app_experiment_detail.tex <==
% !TEX root = main.tex
%\section{Remark for Dirichlet Sampling Algorithms}\label{sec:diri_remark}
%The $i$-th coordinate of the reduced-natural SGRLD iterates read
%\begin{align}
%\y^{k+1}_i = \y^{k}_i - \eta_k  &\Big( G^{-1}(\y^k) \nabla W(\y^k) \Big)_i - 2 \sum_{j=1}^d \l(  G^{-1}(\y^k) \frac{\partial G(\y^k)}{\partial y_j} G^{-1}(\y^k)\r)_{ij}    \nn\\
%&+ \sum_{j=1}^d G^{-1}(\y^k)_{ij} \Tr \l( G^{-1}(\y^k)  \frac{\partial G(\y^k)}{\partial y_j}\r)  + \l(\sqrt{2 \eta_k  G^{-1}(\y^k)} \bm{\xi}^k \r)_i  \label{eq:diri_remark_hold}\\
%\end{align}
%where
%$G^{-1} = \l( \sum_{i=1}^{d=1} n_i\r)\l(   \diag \l( \nabla \hstar \r)^{-1} + \frac{1}{1- \sum_{i=1}^d  \l(\nabla \hstar \r)_i }  \mathbf{1}\mathbf{1}^\top  \r)$. Even though the reduced-natural SGRLD uses the same variable transformation (i.e., $\x^k = \nabla \hstar (\y^k)$ ), the A-MLD is quite different from the SGRLD in the reduced-natural parametrization.
\section{Experimental Details}\label{app:experiments}

%\subsection{Parameters for Synthetic Data}\label{app:expriment_syn_parameters}




%\subsection{Implementation Details for the Latent Dirichlet Allocation}\label{app:experiment_lda}
In the case of LDA model, one important observation is that two of the latent variables, topic mixtures $\eta \in \mathbb{R}^{D \times K}$ and topic distributions over words $\pi \in \mathbb{R}^{K \times N}$, are essentially matrices. In our experimental setup, we sample from the posterior distribution over the hidden variable $\pi$ where each row $\pi_k$ lies on the probability simplex and all the rows have the same symmetric Dirichlet prior with hyper-parameter $\gamma$. It is also necessary to denote that distribution for each topic is independent from any other. This naturally leads to individual treatment of each row and a simple reformulation of $\nabla h(\bm x), \nabla h^{\star}(\bm y), \nabla^2 h(\bm x)$ and $\nabla^2 h^{\star}(\bm y)$.

Let $\x \in \mathbb{R}^{KN \times 1}$ be the vectorized form of latent topic distribution variable $\pi$ where the vectorization is handled in a row-major fashion.  Given that $\pi_i$ denotes the i\ts{th} row of the matrix $\pi$, $\x$ has the form $[\pi_1, \pi_2, ..., \pi_k]^T$. $\x$ is not a proper probability distribution by itself but each $N$-dimensional block, corresponding to some row of $\pi$, represents a point in probability simplex, following a Dirichlet distribution. Hence, we propose to apply the gradient map $\nabla h$ in a block-wise fashion.

Let $\nabla \tilde{h} : \mathbb{R}^{KN \times 1} \rightarrow \mathbb{R}^{K(N-1) \times 1}$ be the new construction of gradient of the mirror map such that:

\begin{equation}
	\nabla \tilde{h}(\x) = 
	\begin{bmatrix}
		\nabla h(\bm{x}_{1:N}) \\
		\nabla h(\bm{x}_{(N+1):2N}) \\
		\vdots \\
	 	\nabla h(\bm{x}_{(K-1)(N+1):KN})
	\end{bmatrix}
\label{}
\end{equation}

where $\x_{(i-1)(N+1):iN}$ is the i\ts{th} block in $\x$ (or equivalently $\pi_i$). For notational simplicity, we will denote i\ts{th} block of $\x$ as $\x_{B_i}$. Similarly, we follow the same convention for $\nabla \tilde h^{\star}(\bm y)$. It immediately follows that $\nabla \tilde{h} \circ \nabla \tilde h^\star$ yields identity operator as:

\begin{equation}
	\nabla \tilde h \circ \nabla \tilde h^\star (\bm y)
	=
	\begin{bmatrix}
		\nabla h(\bm{x}_{B_1}) \\
		\nabla h(\bm{x}_{B_2}) \\
		\vdots \\
		\nabla h(\x_{B_K})
	\end{bmatrix}
	\circ
	\begin{bmatrix}
		\nabla h^{\star}(\bm y_{B_1}) \\
		\nabla h^{\star}(\bm y_{B_2}) \\
		\vdots \\
		\nabla h^{\star}(\bm y_{B_K})
	\end{bmatrix}
	=
	\begin{bmatrix}
		\nabla h \circ \nabla h^{\star}(\bm y_{B_1}) \\
		\nabla h \circ \nabla h^{\star}(\bm y_{B_2}) \\
		\vdots \\
		\nabla h \circ \nabla h^{\star}(\bm y_{B_K})
	\end{bmatrix}
	=
	\bm y
\label{eq.tilde_h_identity}
\end{equation}

where $\bm y_{B_i}$ denotes the i\ts{th} block of $\bm y \in \mathbb R^{K(N-1) \times 1}$. Note that each block $\bm y_{B_i}$ is of dimension N-1, due to the specific choice of entropic mirror map. The same holds for $\nabla \tilde h^\star \circ \nabla \tilde h$.

Let $e^{-V} \drm \x $ represent the posterior distribution $p(\pi | w, z, \alpha, \gamma)$ up to a certain constant. Due to the particular analytical structure of the posterior distribution, the target distribution $e^{-V(\x)} \drm \x $ can be decomposed as $e^{- \sum_{k=1}^K V_i(\x_{B_k})} \drm \x$, where each component $e^{-V_i(\x_{B_i})} \drm \x$ is a valid Dirichlet posterior distribution. Then we have:%, we claim that $e^{-W_i} \drm \bm y$ is the push-forward measure of $e^{-V_i} \drm \x$ under $\nabla h$.
\begin{lemma}
Let $e^{-W(\bm y)} \drm \bm y$ be the push-forward of $e^{-V(\x)} d \x = e^{- \sum_{k=1}^K V_k(\x_{B_k})} d \x$ under $\nabla \tilde h$. Then
\begin{enumerate}
\item $W$ has a corresponding block-decomposable form \beq W = \sum_{k=1}^K W_k, \eeq where  $e^{-W_k(\bm y_{B_k})} \drm \bm y_{B_k}= \nabla h \# e^{-V_k(\x_{B_k})} \drm \x_{B_k}$.
\item $W$ is convex in $\bm y$.
\end{enumerate}
\label{lem.lda_pushforward}
\end{lemma}

\begin{proof}
	By the assumption $e^{-W(\bm y)} \drm \bm y = \nabla \tilde h \# e^{-V(\x)} \drm \x$, we have, by \eqref{eq:Monge-Ampere},
	\begin{equation}
		e^{-V} = e^{-W \circ \nabla \tilde h} \det \nabla^2 \tilde h
	\end{equation}
	which can be rewritten as
	\begin{align}
		W \circ \nabla \tilde h &= V + \log \det \nabla^2 \tilde h \nn \\
		&= \sum_{k=1}^K V_k + \log \det \nabla^2 \tilde h. \label{eq:experiment_hold1}
	\end{align}
	
	Moreover, $\nabla^2 \tilde h$ is a block-diagonal matrix of the form \beq \diag \Big[\nabla^2 h(\x_{B_1}), \nabla^2 h(\x_{B_2}), ..., \nabla^2 h(\x_{B_K}) \Big] \eeq since cross derivatives of any of the blocks are zero; i.e., for any $i \neq j$, $\frac{\partial}{\partial \x_{B_i} \partial \x_{B_j}}  \tilde h = 0$. Therefore, $\det \nabla^2 \tilde h = \prod_{k=1}^K \det \nabla^2 h(\x_{B_k})$, which implies $\log \det \nabla^2 \tilde h = \sum_{k=1}^K \log \det \nabla^2 h(\x_{B_k})$. Substituting into \eqref{eq:experiment_hold1} yields
	\begin{equation}
		W \circ \nabla \tilde h(\x) = \sum_{k=1}^K \Big( V_k(\x_{B_k}) + \log \det \nabla^2 h(\x_{B_k})  \Big).\\
	\end{equation}
	
	Using Equation \ref{eq.tilde_h_identity} and the fact that $\nabla^2 h \circ \nabla h^\star = {\nabla^2 h^\star}^{-1}$, we get
	\begin{align}
		W &= \sum_{k=1}^K \Big( V_k \circ \nabla h^\star(\bm y_{B_k}) - \log \det \nabla^2  h^\star(\bm y_{B_k}) \Big), \text{ and}\\
		W_k &= V_k \circ \nabla h^\star - \log \det \nabla^2  h^\star
		%e^{-W_k} &= e^{-V_k \circ \nabla h^\star} \det \nabla^2  h^\star \\
		%e^{-V_k} &= e^{-W_k \circ \nabla h} \det \nabla^2  h \\
		%e^{-W_k(\bm y_{B_k})} d \bm y_{B_k} &= \nabla h \# e^{-V_k(\x_{B_k})} d \x_{B_k}
	\end{align}which proves that $\nh \# e^{-V_k} = e^{-W_k}$.
	
	Due to \eqref{eq:dirichlet_dual}, when $e^{-V_k(\x_{B_k})} \drm \x_{B_k}$ is a Dirichlet distribution and $h$ is the entropic mirror map, then $W_k$ is strictly convex and Lipschitz gradient. Therefore, $W$ is convex since it is a sum of convex functions. 
\end{proof}


==> app_fokker_planck.tex <==
\section{Fokker-Planck Equation and Stationary Measure}\label{app:fokker_planck}

We show that: 
\begin{theorem}[Symmetry implies stationarity]
If $\Lh$ is $\mathbb{L}_2$-symmetric with respect to $\mu$:
\beq \nn% \label{eq:app_symmetric}
\int g \Lh f \dmu = \int f \Lh g \dmu \quad \forall f, g \in \Cc,
\eeq
then $\mu$ is a stationary measure for the SDE corresponding to $\Lh$. 
\end{theorem}

The simplest way to see this is to derive the Fokker-Planck equation and identify the stationary measure.

\begin{proof}
Let $p(t,\x)$ be the probability density function of $\X_t$, and let $q(t,\x) = \frac{p(t,\x)}{e^{-V(\x)}}$ be the relative density with respect to $\mu$ at time $t$. For any $f\in \Cc$, we have, by It\^{o}'s lemma,
\beq
f(\X_t) =  f(\X_0) + \int_0^t \Lh f(\X_s)\drm s + \textup{martingale}. \nn
\eeq
Taking expectation and using Fubini's theorem, we obtain
\beq \nn
\EE f(\X_t) = \EE f(\X_0) + \int_0^t \EE[ \Lh f(\X_s)] \drm s 
\eeq
which reads
\begin{align}
\int f(\x)q(t,\x)\dmu(\x) &= \int f(\x)q(0,\x)\dmu(\x) + \int_0^t \int  \Lh f(\x) q(t,\x)   \dmu(\x) \drm s \nn\\
&= \int f(\x)q(0,\x)\dmu(\x) + \int_0^t \int  f(\x) \Lh q(t,\x)   \dmu(\x) \drm s \label{eq:app_fp_hold1}
\end{align}where the second equality uses the fact that $\Lh$ is symmetric with respect to $\mu$. Since \eqref{eq:app_fp_hold1} holds for all $f \in \Cc$, we conclude that
\beq
q(t,\x) = q(0,\x) +\int_0^t \Lh q(s, \x)\drm s. \nn
\eeq
Taking the time derivative, we see that $q$ must satisfy 
\beq
\frac{\partial q}{\partial t}  = \Lh q. \nn
\eeq
Therefore, if $\Lh q(0, \cdot) = 0$, which is obviously satisfied by $q(0,\cdot)\equiv 1$ (i.e., $\X_0 \sim \mu$), then $q(t,\cdot) \equiv 1$ for all $t$, implying that $\mu$ is a stationary measure.
\end{proof}

==> app_ricci.tex <==
\section{Expressions for the Bakry-Emery Tensor} \label{app:ricci}
See \citep{kolesnikov2014hessian} for omitted details in this appendix. 

Let $\mathbf{H}$ be the matrix whose $(i,j)$-th entry is
\beq \nn
H_{i,j} = \Tr \left[ \l(\nabla^2 h\r)^{-1} \nabla^2 \l( \partial_i h  \r) \l(\nabla^2 h\r)^{-1} \nabla^2\l(\partial_j h \r) \right].
\eeq 
Then $\mathbf{H} \succeq \frac{1}{d} \nabla \log\det \nabla^2 h \otimes \nabla \log \det \nabla^2 h \succeq 0$.

The Bakry-\'Emery tensor for the manifold $(\RR^d, \nabla^2 h, \mu)$ is given by 
\begin{align} %\label{eq:bakry_emery_tensor}
\Ricg &\coloneqq \frac{1}{4}\mathbf{H} + \frac{1}{2} \Big( \nabla^2 V + \nabla^2 h \cdot\l( \nabla^2W \circ \nabla h \r) \cdot \nabla^2 h \Big) \nn \\
&= \nabla^2 V + \frac{1}{2} \nabla^2 \log\det \nabla^2 h + \frac{1}{4} \mathbf{H} - \frac{1}{2} \sum_{i=1}^d \ip{(\nabla^2h)^{-1}\l( \nabla V + \nabla \log\det\nabla^2 h \r)}{\mathbf{e}_i} \nabla^2 (\partial_i h). \nn
\end{align}

==> app_s-mld.tex <==
\section{Proof of \textbf{Theorem \ref{thm:s-mld}}}\label{app:s-mld}
\begin{enumerate}
\item  We consider the coupled dynamics
\beq \label{eq:app_smd_dynamics}
   \left\{
                \begin{array}{ll}
                  \drm\Y_t = -\nabla V(\X_t) \dt+ \sqrt{2 \nabla^2 h(\X_t)} \dBt\\
                  \X_t = \nabla \hstar (\Y_t)
                \end{array}.
              \right.
  \eeq
To see that \eqref{eq:app_smd_dynamics} is equivalent to 
\beq \label{eq:app_smld_hold1}
\drm \X_t = - (\nabla W \circ \nabla h) (\X_t)\dt + \sqrt{2\nabla^2 h(\X_t)^{-1}}\dBt,
\eeq
we apply It\^o's lemma to any function $f \in\Cc$ in \eqref{eq:app_smld_hold1} and get
\begin{align}
\drm f(\X_t) &=  \left\{   \Tr \nabla^2 h(\X_t)^{-1} \nabla^2 f - \ip{\nabla W \circ \nabla h} { \nabla f} \right\} \dt+ \nabla f(\X_t)^\top \sqrt{2\nabla^2 h(\X_t)^{-1}}\dBt \nonumber \nn\\
&= \Lh f(\X_t) \dt + \nabla f(\X_t)^\top \sqrt{2\nabla^2 h(\X_t)^{-1}}\dBt \label{eq:app_smld_hold2}
\end{align}
by \eqref{eq:diffusion_equivalent1}. Now, substituting $ f\leftarrow\partial_i h $ in \eqref{eq:app_smld_hold2} and using \eqref{eq:Lh_differential_equation}, we see that 
\begin{align*}
\drm\Y_t = \drm\nh(\X_t)&=  -\nabla V(\X_t) \dt+ \nabla^2 h(\X_t) \sqrt{2\nabla^2 h(\X_t)^{-1}}\dBt \\
&= -\nabla V(\X_t) \dt + \sqrt{2\nabla^2 h(\X_t)}\dBt 
\end{align*}
which establishes 1 of \textbf{Theorem \ref{thm:s-mld}}.
\item The claims follow from \eqref{eq:app_smld_hold2}, and 1, 2 of \textbf{Lemma \ref{lem:properties_Lh}}.
\item Since $\Y_t = \nh (\X_t)$, we have 
\begin{align}
\nabla^2 h(\X_t) &= (\nabla^2 h \circ \nhstar) (\Y_t) \nn \\
&= \nabla^2 \hstar (\Y_t)^{-1}. \label{eq:app_smld_hold3}
\end{align} 
Plugging \eqref{eq:app_smld_hold3} into \eqref{eq:app_smd_dynamics} establishes the claim.
\item This is a direct consequence of the classical Fenchel duality $(\nh \circ \nhstar )(\x) = \x$. Simply reverse the role of $\X_t$ and $\Y_t$ in the proof of part 1 and use $\nh \leftarrow \nhstar$ to redo the analysis.
\end{enumerate}



==> app_smld_nips.tex <==
\section{Symmetric Langevin Dynamics} \label{app:s_mld_nips}


\subsection{Weighted Divergence, Weighted Laplacian, and Generators}\label{subsec:weighted}
\subsubsection{Weighted Divergence}
Given a probability measure $\nu$ and a smooth vector field $\psi: \RR^d \rightarrow \RR^d$, the \textbf{weighted divergence} operator $\Div_\nu$%, sending $\psi$ to a real-valued function $\Div_\nu \psi : \RR^d \rightarrow \RR$, 
~is defined as the formal (negative) $\mathbb{L}_2$-adjoint of the gradient operator with respect to $\nu$:
\beq \label{eq:weighted_divergence}
\int \ip{\nabla f  }{\psi} \drm\nu = -\int f \Div_\nu \psi \drm\nu \quad \forall f \in \Cc.
\eeq 
Several equivalent formulations of $\Div_\nu$ are given in \textbf{Appendix \ref{app_weighted_divergence}}.

If $\nu$ is the Lebesgue measure, then $\Div \psi= {\Sigma}_{i=1}^d \frac{\partial \psi_i}{\partial x_i}$, where $\psi_i$ is the $i$-th coordinate of the vector-valued function $\psi$.

\subsubsection{Weighted Laplacian}
Given a probability measure $\nu$ and a function $f \in \Cc$, the \textbf{weighted Laplacian} operator $\Delta_\nu$ sends $f$ to a real-valued function $\Delta_\nu f$ by the formula
\beq \label{eq:weighted_laplacian}
\Delta_\nu f  =  \Div_\nu \l(  \nabla f  \r).
\eeq
In particular, we have the integration by parts for every $f, g \in \Cc$ (see \textbf{Appendix \ref{app_weighted_laplacian}}):
\beq \label{eq:integration_by_parts}
\int \ip{\nabla f  }{\nabla g} \dnu = -\int f \Delta_\nu g \dnu = -\int g \Delta_\nu f \dnu,
\eeq
which shows that every operator of the form \eqref{eq:weighted_laplacian} is \textbf{symmetric} in $\mathbb{L}_2$ with respect to $\nu$. %Formally, we say that $\Delta_\nu = \Div_\nu \circ \nabla$. 
Equivalent formulations of $\Delta_\nu$ may be found in \textbf{Appendix \ref{app_weighted_laplacian}}.

If $\nu$ is the Lebesgue measure, then $\Delta = \Sigma_{i=1}^d \frac{\partial^2}{\partial x^2_i}$ is the Euclidean Laplacian operator.

\subsubsection{Generators}\label{subsec:generator}
Consider the $d$-dimensional stochastic differential equation (SDE) below, known as the (time-homogeneous) It\^o's diffusion:
\beq \label{eq:ito_diffusion}
\drm\X_t = b(\X_t)\dt + \sqrt{2} \sigma(\X_t)\dBt,
\eeq
where $b: \RR^d \rightarrow \RR^d$ and $\sigma: \RR^d \rightarrow \RR^{d\times d}$. By It\^o's lemma \citep{oksendal2003stochastic}, for any $f \in \Cc$, we have
\beq \label{eq:ito_lemma}
\drm f(\X_t) =  \l( \ip{b(\X_t)}{\nabla f(\X_t)}  + \Tr \sigma(\X_t)\sigma(\X_t)^\top \nabla^2 f(\X_t) \r) \dt + \sqrt{2}\nabla f(\X_t)^\top \sigma(\X_t)\dBt.
\eeq
The \textbf{generator} $\mathcal{L}$ of \eqref{eq:ito_diffusion}, acting on functions $f\in \Cc$, is the $\dt$ term in \eqref{eq:ito_lemma}:
\beq \label{eq:generator_sde}
\mathcal{L}f \coloneqq  \Tr \sigma\sigma^\top \nabla^2 f + \ip{b}{\nabla f}.
\eeq
%It is well-know that $\mathcal{L}$ determines the stationary measure \citep{bakry2013analysis}. 
The Langevin Dynamics \eqref{eq:langevin_dynamics} has generator $\mathcal{L} f = \Tr \nabla^2 f - \ip{\nabla V}{\nabla f} = \Delta f - \ip{\nabla V}{\nabla f}$. An equivalent formulation (see \textbf{Appendix \ref{app_weighted_generator}}) is $\mathcal{L} f = \Div_\mu (\nabla f)$ where $\dmu = \dV$, and hence, $\Lcal$ is $\mathbb{L}_2$-symmetric with respect to $\mu$.

\section{Symmetric Mirrored Langevin Dynamics}\label{sec:smld}
In Section \ref{subsec:smld}, we consider the first candidate of sampling from mirror descent-type dynamics. Continuous convergence rates are given in Section \ref{subsec:conv}, and a negative example to discretization is presented in Section \ref{subsec:disc_S-MLD}.

\subsection{Symmetric Mirrored Langevin Dynamics: Motivation and Derivation}\label{subsec:smld}
The classical (stochastic) mirror descent dynamics for optimizing $V$ is given by \citep{raginsky2012continuous, krichene2015accelerated, mertikopoulos2018convergence}
\beq \nn%\label{eq:mirror_descent_dyanmics}
   \left\{
                \begin{array}{ll}
                  \drm \Y_t = -\nabla V(\X_t) \dt + \sqrt{2} \sigma(t)\dBt  \\
                  \X_t = \nabla \hstar (\Y_t)
                \end{array}
        \right. 
\eeq
where $\sigma(t) \in \RR^+$. For sampling from $\dmu \coloneqq \dV$, it is then natural to posit a dynamics of the form
\beq \label{eq:symmetric-mirror_descent_dyanmics}
   \left\{
                \begin{array}{ll}
                  \drm \Y_t = -\nabla V(\X_t) \dt + \sqrt{2} \sigma(\X_t) \dBt\\
                  \X_t = \nabla \hstar (\Y_t)
                \end{array}
        \right. 
\eeq
where $\sigma : \RR^d \rightarrow \RR^{d\times d}$ is to be chosen such that the stationary distribution of $\X_t$ is $\mu$. %It is clear that in general, $\sigma$ must depend on $h$, since otherwise whatever works for $h$ would not work for $h \leftarrow 2h$.  


Identifying the correct form of $\sigma$ involves more sophisticated generator theory than the Langevin Dynamics. To see this, let $\Lh$ be the generator of the SDE governing $\drm \X_t$. By \eqref{eq:generator_sde} and \eqref{eq:symmetric-mirror_descent_dyanmics}, we must have
\beq \label{eq:Lh_pde}
\partial_i V = - \Lh \l(\partial_i h\r)
\eeq
for all $i = 1, 2, ..., d.$ There are potentially infinitely many $\Lh$'s satisfying \eqref{eq:Lh_pde}, but they may not give rise to the target stationary distribution $\mu$. Therefore, we further require $\Lh$ to be \textbf{symmetric} in $\mathbb{L}_2$ with respect to $\mu$:
\beq \label{eq:L2_symmetry}
\int f \Lh g \dmu = \int g\Lh f \dmu \quad \quad \forall f, g \in \Cc.
\eeq
It is well-known that (see \textbf{Appendix \ref{app:fokker_planck}}) the corresponding SDE would have the desired stationary distribution $\X_\infty \sim \mu$. 


We now speculate a formula for $\Lh$ that simultaneously satisfies \eqref{eq:Lh_pde} and \eqref{eq:L2_symmetry}. Letting $g \leftarrow \partial_i h$ in \eqref{eq:L2_symmetry}, we get, by \eqref{eq:Lh_pde},
\begin{align}
\int f \Lh \l( \partial_i h\r) \dmu &= \int f \l( -\partial_i V\r) \dmu \nn\\
&= \int f(\x) \partial_i \l(  e^{-V(\x)}  \r) \dx \nn\\
&= -\int \partial_i f\dmu \label{eq:symmetric_hold1}
\end{align}by integration by parts. On the other hand, by \eqref{eq:L2_symmetry}, we may equivalently evaluate \eqref{eq:symmetric_hold1} as:
\begin{align}
\int f \Lh \l( \partial_i h\r) \dmu &= \int \l(\Lh f  \r) \cdot  \l(\partial_i h\r) \dmu \nn \\
&= \int \Big( \l(\Lh f  \r) \circ \nhstar (\y) \Big) \cdot y_i \dnu (\y), \quad \nu \coloneqq \nh \# \mu \label{eq:symmetric_hold2}
\end{align}
by \eqref{eq:push_forward}. To enforce \eqref{eq:symmetric_hold2} = \eqref{eq:symmetric_hold1}, we then conjecture the following form for $\Lh$:
 \beq \label{eq:generator_h}
\Lh f =  \Div_{\nu}\l(  \nabla f\circ \nhstar  \r) \circ \nh  \quad \ \ \  \forall f \in \Cc.
\eeq
Indeed, substituting \eqref{eq:generator_h} into \eqref{eq:symmetric_hold2} gives, with $\mathbf{e}_i$ denoting the $i$-th standard basis of $\RR^d$,
\begin{align*}
\int \Big( \l(\Lh f  \r) \circ \nhstar (\y) \Big) \cdot y_i \dnu (\y) &= \int \Div_\nu \l( \nabla f \circ \nhstar (\y) \r) \cdot y_i \dnu (\y) \\
&= -\int \ip{ \nabla f \circ \nhstar   }{\mathbf{e}_i} \dnu  && \text{by \eqref{eq:weighted_divergence}} \\
&= -\int \ip{\nabla f} {\mathbf{e}_i} \dmu && \text{by \eqref{eq:push_forward}} \\
&= -\int \partial_i f\dmu  = \eqref{eq:symmetric_hold1}.
\end{align*}%which is equal to 
%
%{\color{red}
% in the spirit of Langevin Dynamics, let us look for a $\mathbb{L}_2$-\textbf{symmetric} generator $\Lh$ for $\X_t$ with respect to $\mu$, meaning 
%
%
%Since we have used $\nh$ to couple the dynamics between $\X_t$ and $\Y_t$ in \eqref{eq:symmetric-mirror_descent_dyanmics}, by \textbf{Theorem \ref{thm:coupling}} the pair $(\X_t, \Y_t)$ must confine $\nh \# \X_t = \Y_t$ for all $t > 0$, and in particular we must have $\Y_\infty \sim \nu = \dW \coloneqq\nh \# \mu$. Recalling that the symmetric generator for the Langevin Dynamics of $\mu$ is $\Lcal_\mu f= \Div_{\mu}(\nabla f)$, it is natural to seek for a generator $\Lh$ of the form
%
%That is, we map $\X_t$ to $\Y_t$ using $\nh$, diffuse in such a way that the stationary distribution is $\nu$, and map $\Y_t$ back to $\X_t$ using $\nhstar$.
% }

Incidentally, the odd-looking $\Lh$ in \eqref{eq:generator_h} had recently appeared in the context of {Weighted Hessian Manifolds} \citep{kolesnikov2014hessian}, with a completely different motivation and interpretation. There, the object of interest is the triplet $(\RR^d, \nabla^2 h, \mu)$, viewed as a Riemannian manifold, and the operator $\Lh$ is obtained by differentiating the Monge-Amp\`ere equation \eqref{eq:Monge-Ampere}.% in the $i$-th coordinate. 
~The SDE perspective in this paper, in particular the mirror-descent interpretations, did not appear in \citep{kolesnikov2014hessian}.

Invoking the theory in \citep{kolesnikov2014hessian}, we prove that the correct $\sigma$ in \eqref{eq:symmetric-mirror_descent_dyanmics} is \\$\sigma(\X_t) = \sqrt{\nabla^2 h(\X_t)}$, supported by  several elegant primal-dual structures.

%Crucially, in \citep{kolesnikov2014hessian}, $\Lh$ is shown to obey certain differential equations, which turns out to be exactly what we need to determine the correct $\sigma$ in \eqref{eq:symmetric-mirror_descent_dyanmics}.
\begin{theorem}[Symmetric Mirror Langevin Dynamics]\label{thm:s-mld}
Let $\dmu = \dV$ and $h$ be strictly convex, and denote the pushed-forward measure by $\dnu = \dW \coloneqq \nh \# \dmu.$ Then
\begin{enumerate}
\item Let $\sigma(\X_t) = \sqrt{\nabla^2 h(\X_t)}$ in \eqref{eq:symmetric-mirror_descent_dyanmics}. Then the SDE governing $\X_t$ is
\beq
\drm \X_t = - (\nabla W \circ \nh )(\X_t)\dt + \sqrt{2\nabla^2 h(\X_t)^{-1}} \dBt. \label{eq:sde_X}
\eeq
\item Let $\Lh$ be as given in \eqref{eq:generator_h}. Then $\Lh$ is the generator for \eqref{eq:sde_X}. Moreover, $\Lh$ is symmetric in $\mathbb{L}_2$ with respect to $\mu$, and hence the stationary measure of $\X_t$ is $\X_\infty \sim \mu$.
\item Dually, the SDE governing $\Y_t$ can be written as 
\beq
\drm \Y_t = -(\nabla V \circ \nhstar) (\Y_t) \dt + \sqrt{2\nabla^2 h^\star(\Y_t)^{-1}} \dBt. \label{eq:sde_Y}
\eeq
\item The generator for \eqref{eq:sde_Y} is $\mathcal{L}_{\hstar}$. Moreover, $\Lcal_\hstar$ is symmetric in $\mathbb{L}_2$ with respect to $\nu$, and hence the stationary measure of $\Y_t$ is $\Y_\infty \sim \nu$.
\end{enumerate}
\end{theorem}
\begin{proof}
See \textbf{Appendix \ref{app:s-mld}}.
\end{proof}

\subsection{Continuous Convergence of Symmetric Mirrored Langevin Dynamics}\label{subsec:conv}
Continuous convergence of \eqref{eq:sde_X} depends jointly on $V$ and $h$, but in a rather tangled fashion. The purpose of this subsection is to seek for simple sufficient conditions for deriving convergence rates. To this end, we will leverage one more property of $\Lh$: It is the generator of a diffusion process on the Weighted Hessian Manifold $(\RR^d, \nabla^2 h, \mu)$ \citep{kolesnikov2014hessian}.

The original motivation of \citet{kolesnikov2014hessian} for studying $\Lh$ is to compute an explicit form for the \textbf{Bakry-\'Emery tensor} in the above-mentioned manifold. A far-reaching result of \citet{bakry1985diffusions} states that the {continuous convergence} of the diffusion processes is intimately related to the Bakry-\'{E}mery tensor. Leveraging this well-established theory, convergence analysis for \eqref{eq:sde_X} admits a simple reduction to existing results.
\begin{theorem}[Convergence Rates of Symmetric Mirrored Langevin Dynamics]\label{thm:convergence_conti_mld}
Let $\dmu = \dV$ be the target distribution and $h$ be a strictly convex mirror map. Let $\Ricg$ be any of the expressions given in \textbf{Appendix~\ref{app:ricci}}. If $\Ricg \succeq \rho \nabla^2h$ for some $\rho >0$, then $\X_t\sim \mu_t$ converges exponentially to $\X_\infty \sim \mu$ in total variation distance:
\beq \label{eq:convergence_S-MLD_TV}
\dTV(\mu_t, \mu) \leq \frac{1}{2} \sqrt{\chi^2(\mu_0, \mu)} \cdot e^{-\frac{\rho t}{2}}
\eeq
where $\chi^2(\mu_0, \mu)  \coloneqq \int \l(  \frac{\dmu_0}{\dmu}(\x) -1 \r)^2 \dmu(\x)$ is the $\chi^2$-divergence.
\end{theorem}
\begin{proof}
The proof is essentially due to \citet{dalalyan2017theoretical}; see \textbf{Appendix~\ref{app:proof_convergence_smld}}.
\end{proof}
\begin{remark}
{It should be noted that \citet{dalalyan2017theoretical} already noticed the link between Bakry-\'Emery theory and continuous convergence of Langevin Dynamics. The connection between S-MLD and Bakry-\'Emery theory generalizes beyond this special case.}
\end{remark}
%
%\begin{theorem}[Convergence Rate under the Curvature-Dimension Condition]\label{thm:convergence_conti_mld}
%Let $X_0 \sim \mu_0$. Suppose blah. Then we have
%\beq \label{eq:convergence_conti_mld}
%\|   P^\star_t \mu_0 - \mu \|_{\textup{TV}} \leq  \frac{1}{2}\chi^2(\mu_0, \mu) e^{-\rho{t}}
%\eeq
%where 
%\end{theorem}

%\begin{lemma}[Bakry-Em\'{e}ry Ricci Tensor for Entropic Mirror Map]
%Let $h(\x) = \sum_{i=1}^d x_i \log x_i$. Then 
%\beq
%\Ricginf (\x)= \nabla^2 V (\x)+ \frac{1}{4} [x_i^{-2}]_i + \frac{1}{2} \left[\frac{(\nabla V(\x))_i}{x_i}\right]_i.
%\eeq
%\end{lemma}


\subsection{A Negative Example to Discretizing Mirrored Langevin Dynamics}\label{subsec:disc_S-MLD}
We discuss the practicality of the S-MLD by applying (time-wise) discretization to \eqref{eq:sde_X}. Our main observation is the following negative example:
\begin{theorem}[CIR Processes and Symmetric Mirrored Langevin Dynamics] \label{thm:negative_example}
There exist strictly convex $V$ and $h$ such that the SDE \eqref{eq:sde_X} reduces to the Cox–Ingersoll–Ross (CIR) processes \eqref{eq:cir_process}.
\end{theorem}
\begin{proof}
See \textbf{Appendix \ref{app:cir}}.
\end{proof}
The CIR process is an influential short rate model for describing the evolution of interest rates \citep{cox1985theory}. Unfortunately, discretized CIR processes are known to exhibit slow (logarithmic) convergence, both in theory \citep{gyongy2011note} and practice \citep{alfonsi2005discretization}. Although this can be partially remedied by more sophisticated discretization schemes \citep{kloeden2013convergence}, the example in \textbf{Theorem \ref{thm:negative_example}} indicates the absence of a satisfactory framework to obtaining general convergence guarantees, even in the case of strictly convex $V$ and $h$.



==> app_weighted_divergence.tex <==
\section{Weighted Divergence, Weighted Laplacian, and Generators}\label{app_weighted}
All materials in Section \ref{subsec:weighted} are classical, but we cannot find a proper literature. The proofs are provided for completeness.

We need the (Euclidean) divergence formula, which is a generalization of the product rule to higher dimension:
\beq \label{eq:divergence_formula}
\Div (f \psi) = \ip{\nabla f}{\psi} + f\Div\psi, \quad \forall f \in \Cc, \psi \textup{ a smooth vector field}
\eeq
where $\Div \psi = \sum_{i=1}^d \frac{\partial \psi_i}{\partial x_i}.$
We also need the integration by parts for the Euclidean divergence:
\beq \label{eq:integration_by_parts_euclidean}
\int \ip{\nabla f}{\psi} \dx = - \int f \Div \psi \dx \quad \forall f\in \Cc, \psi \text{ a smooth vector field}
\eeq
which is simply obtained by integrating both sides of \eqref{eq:divergence_formula}, invoking the Stokes' theorem on the left-hand side, and using that $f$ is compactly supported.

\subsection{Equivalent Formulations of $\Div_\nu$}\label{app_weighted_divergence}
\begin{theorem}The weighted divergence in \eqref{eq:weighted_divergence} may be characterized as:
\begin{align}
\Div_\nu \psi &= e^{W} \Div (e^{-W}\psi) \label{eq:weighted_divergence_formula1} \\
 &= \Div\psi-\ip{\nabla W}{\psi}. \label{eq:weighted_divergence_formula2}
\end{align}
\end{theorem}
\begin{proof}
We will only prove \eqref{eq:weighted_divergence_formula1} = \eqref{eq:weighted_divergence_formula2} $\Rightarrow$ \eqref{eq:weighted_divergence}. The uniqueness of $\Div_\nu$ requires approximation arguments that are beyond the interest of this paper.

For any $f\in \Cc$, we have, by \eqref{eq:integration_by_parts_euclidean}, 
\begin{align*}
\int f e^{W} \Div (e^{-W}\psi) \dnu &= \int f \Div(e^{-W}\psi) \dx \\
&= -\int \ip{\nabla f}{ \psi } e^{-W(\x)}\dx \\
&= -  \int \ip{\nabla f}{ \psi } \dnu
\end{align*}which proves \eqref{eq:weighted_divergence}. On the other hand, using \eqref{eq:divergence_formula}, we get 
\beq \nn
e^{W} \Div (e^{-W}\psi) = e^W \l( -e^{-W}  \ip{\nabla W}{ \psi} + e^{-W} \Div \psi\r)
\eeq 
which is \eqref{eq:weighted_divergence_formula2}.
\end{proof}

\subsection{Equivalent Formulations of $\Delta_\nu$}\label{app_weighted_laplacian}
\begin{theorem}The weighted Laplacian in \eqref{eq:weighted_laplacian} may be characterized as:
\begin{align}
\Delta_\nu f = \Div_\nu(\nabla f) = \Delta f - \ip{\nabla W}{ \nabla f}. \label{eq:weighted_dlaplacian_formula}
\end{align}Moreover, the integration-by-parts formula \eqref{eq:integration_by_parts} hold.
\end{theorem}
\begin{proof}
Substituting $\psi \leftarrow \nabla f$ in \eqref{eq:weighted_divergence_formula2} and using $\Div \circ \nabla = \Delta$ establishes the first claim. To see \eqref{eq:integration_by_parts}, use \eqref{eq:weighted_dlaplacian_formula} and the fact that $\Div_\nu$ is the (negative) $\mathbb{L}_2$-adjoint of $\nabla$ with respect to $\nu$.
\end{proof}

\subsection{Equivalent Formulations of $\mathcal{L}$ for Langevin Dynamics}\label{app_weighted_generator}
\begin{theorem}
The generator of the Langevin Dynamics corresponding to $\dmu = \dV$ can be equivalently characterized as
\begin{align}
\Lcal f = \Div_\mu (\nabla f) = \Delta f - \ip{\nabla V}{\nabla f}.
\end{align}
\end{theorem}
\begin{proof}
This is simply \eqref{eq:weighted_dlaplacian_formula} with $\nu \leftarrow \mu$ and $W \leftarrow V$.
\end{proof}


==> conclusion.tex <==
% !TEX root = main.tex
\section{Conclusion and Future Work}
%We initiate a study of the Langevin Dynamics in the spirit of mirror descent. Our theory of A-MLD improves the state-of-the-art rates for compactly supported distributions. On the simplex, the SMLD promises practical algorithms with rigorous guarantees.
%
%Two questions naturally arise in our theory. First, for strong convexity of the entropy, we have used the crude bound $\| \cdot\|_1 \geq \| \cdot\|$. We defer the work to fully exploit the $\ell_1$-norm in order to sharpen the convergence rates for future. Second, the Dirichlet posterior is but one instance where we can solve the Monge-Amp\`ere equation explicitly. We look forward to seeing more such examples.

==> hold.tex <==
\section{Temporary Stuff}
\eq{
\nabla \log \det \nabla^2 h(\x) &= g^{ij}h_{ijk} \nonumber \\
&= g_{kl}g^{kl}g^{ij}h_{ijk} \nonumber\\
&= 2g_{kl}g^{ij}\Gamma_{ij}^l  \label{eq:holdd1}
}

\eqref{eq:holdd1}
Since $-V = -W \circ \nabla h + \log\det \nabla^2 h$,
\eq{
-\nabla V = -\nabla^2 h \l(  \nabla W \circ \nabla h -  \nabla^2 h^{-1} \nabla \log\det \nabla^2h \r).
}

The Riemannian Brownian motion is given by
\eq{
d\tilde{B_t} &= \sqrt{\nabla^2 h^{-1}} dB_t - \frac{1}{2}g^{ij}\Gamma_{ij}^k dt \\
&= \sqrt{\nabla^2 h^{-1}} dB_t - \frac{1}{4} \nabla^2 h^{-1}\nabla \log \det \nabla^2 h dt,
}
whence
\eq{
dX_t &= -\nabla W \circ \nabla h + \sqrt{2} \nabla^2 h^{-1} dB_t \\
&= - \l( \nabla W \circ \nabla h  -  \nabla^2 h^{-1} \nabla \log\det \nabla^2h\r) + \sqrt{2} \l( \nabla^2 h^{-1} dB_t - \frac{1}{4} \nabla^2 h^{-1}\nabla \log \det \nabla^2 h\r)
}

==> primal-dual_dynamics_conti.tex <==
%\section{Failure of a Na\"ive Guess: The Symmetric- Mirrored Langevin Dynamics}\label{sec:failure}
%The classical mirror descent dynamics is 
%
%
%We first consider a na\"ive integration of a Brownian motion term into the classical mirror descent dynamics:
%\beq \label{eq:mirror_descent_dyanmics}
%   \left\{
%                \begin{array}{ll}
%                  \drm\Y_t = -\nabla V(\X_t) \dt + \sqrt{2} \sigma(\X_t) \dBt\\
%                  \X_t = \nabla \hstar (\Y_t)
%                \end{array},
%        \right.
%\eeq
